Towards Flexible Wireless Charging for Medical Implants Using Distributed Antenna System

This paper presents the design, implementation and evaluation of In-N-Out, a software-hardware solution for far-field wireless power transfer. In-N-Out can continuously charge a medical implant residing in deep tissues at near-optimal beamforming power, even when the implant moves around inside the human body. To accomplish this, we exploit the unique energy ball pattern of distributed antenna array and devise a backscatter-assisted beamforming algorithm that can concentrate RF energy on a tiny spot surrounding the medical implant. Meanwhile, the power levels on other body parts stay in low level, reducing the risk of overheating. We prototype In-N-Out on 21 software-defined radios and a printed circuit board (PCB). Extensive experiments demonstrate that In-N-Out achieves 0.37~mW average charging power inside a 10~cm-thick pork belly, which is sufficient to wirelessly power a range of commercial medical devices. Our head-to-head comparison with the state-of-the-art approach shows that In-N-Out achieves 5.4$\times$--18.1$\times$ power gain when the implant is stationary, and 5.3$\times$--7.4$\times$ power gain when the implant is in motion.

==> Body/abs.tex <==
\subsection*{Abstract}
This paper presents the design, implementation and evaluation of \systemname, a software-hardware solution for far-field wireless power transfer.
\systemname can continuously charge the medical implant residing in deep tissues with consistently near-optimal power, even when the implant moves around inside the human body.
To accomplish this, we exploit the structure of a distributed antenna array and devise a backscatter-assisted beamforming algorithm that can  concentrate RF energy on a tiny spot surrounding the medical implant. Meanwhile, we can keep radiation exposure levels on other body parts very low, reducing the risk of overheating.
We prototype \systemname on 21 software-defined radios and a printed circuit board (PCB).
Through extensive experimentation, we show that \systemname achieves 0.37~mW average charging power inside a 10~cm-thick pork belly, which is sufficient to wirelessly power a range of commercial medical devices from outside the body.
Our head-to-head comparison with the state-of-the-art approach shows that \systemname achieves 5.4$\times$--18.1$\times$ power gain when the implant is stationary, and 5.3$\times$--7.4$\times$ power gain when the implant is in motion.








==> Body/case_study.tex <==
\section{Case Study}
\label{s:case}

In this section, we conduct two case studies to demonstrate how \systemname can be used to provide ubiquitous sensing anywhere at anytime.
In the first case study, we integrate a humidity sensor and a light sensor on the \systemname node, and deploy three of them on the Terracotta Army museum, an indoor place for environment sensing.
In the second case study, we integrate a humidity sensor and a temperature sensor on the \systemname node and mount it on the Golden monkey, the country grade one protected animal, for the field living environment sensing. 

\subsection{Cultural relics preservation}.

The humidity and the light conditions play a key role in the cultural relics preservation.
An improper humidity and light condition would accelerate the surface paint oxidation, and thus destroy the terracotta sculpture.
To monitor the environment, the traditional way is to deploy battery\hyp{}based sensors around these sculptures, which has a limited transmission range and requires a frequent battery replacement.
We replace these battery\hyp{}based sensors with our \systemname node and mount three of them on the sculptures for the humidity and the light condition monitoring, as shown in Figure~\ref{}.

Each \systemname node regularly sends its sensing data, including the real\hyp{}time humidity and the light intensity readings to the gateway \rev{xx}~m away every $N$ minutes.
We vary $N$ and test the maximum transmission rate can be achieved by each node.
As shown in Table~\ref{}, 

\subsection{Wildlife monitoring}.

Wildlife monitoring is of great importance to keeping track of habitat of wild animals.
In this case study, we mount three \systemname node on the Golden monkey to track their living environment in the field. Figure~\ref{} shows the experiment field.
The \systemname node harvests energy from the ambient light and regularly reports the temperature and humidity readings to the gateway.


In the future, we envision to place the gateway on the unmanned aerial vehicle (UAV)  to track the animal movement and group formulation.
This can be achieved by leveraging state\hyp{}of\hyp{}the\hyp{}art wireless localization algorithms such as MUSIC~\cite{xiong2013arraytrack} and JADE~\cite{kotaru2015spotfi}.
